Accuracy-Time Tradeoffs in AI-Assisted Decision Making under Time Pressure

In settings where users both need high accuracy and are time-pressured, such as doctors working in emergency rooms, we want to provide AI assistance that both increases decision accuracy and reduces decision-making time. Current literature focusses on how users interact with AI assistance when there is no time pressure, finding that different AI assistances have different benefits: some can reduce time taken while increasing overreliance on AI, while others do the opposite. The precise benefit can depend on both the user and task. In time-pressured scenarios, adapting when we show AI assistance is especially important: relying on the AI assistance can save time, and can therefore be beneficial when the AI is likely to be right. We would ideally adapt what AI assistance we show depending on various properties (of the task and of the user) in order to best trade off accuracy and time. We introduce a study where users have to answer a series of logic puzzles. We find that time pressure affects how users use different AI assistances, making some assistances more beneficial than others when compared to no-time-pressure settings. We also find that a user's overreliance rate is a key predictor of their behaviour: overreliers and not-overreliers use different AI assistance types differently. We find marginal correlations between a user's overreliance rate (which is related to the user's trust in AI recommendations) and their personality traits (Big Five Personality traits). Overall, our work suggests that AI assistances have different accuracy-time tradeoffs when people are under time pressure compared to no time pressure, and we explore how we might adapt AI assistances in this setting.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

ACMCPSAMPLES= \
	samples/sample-acmcp-Discussion.pdf \
	samples/sample-acmcp-Invited.pdf \
	samples/sample-acmcp-Position.pdf \
	samples/sample-acmcp-Research.pdf \
	samples/sample-acmcp-Review.pdf \

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: ${ACMCPSAMPLES} acmart.cls
	zip $@ $+

samples/sample-acmcp.tex: samples/samples.ins samples/samples.dtx
	cd samples; pdflatex samples.ins; cd ..


samples/sample-acmcp-%.tex: samples/sample-acmcp.tex samples/acm-jdslogo.png
	sed 's/acmArticleType{Review}/acmArticleType{$*}/' $< > $@

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 2.01   \acmPrice now produces a warning.

Version 2.00   ACM switches to electronic only version.
	       We do not print article tabs anymore.
	       New copyright wording.
	       Deleted \acmPrice.

Version 1.93   Added PACMSE

Version 1.92   Documentation update
	       Emergency change: changed order of hyperref and hyperxmp
	       due to changes in the undelying packages

Version 1.91   Minor changes in ACMCP format

Version 1.90a  Changes in the sample keywords and concepts

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> sections/old-3-hypotheses.tex <==
\section{Hypotheses}
\label{sec:hypotheses}

\begin{enumerate}
    \item Participants use different AI assistance types differently under time pressure compared to under no time pressure.
    \begin{enumerate}
        \item On AI-before, people overrely more under time pressure.
    \end{enumerate}
    
    \item Pure vs mixed is different: impacts overreliance rate (scarcity effect was about reliance, not overreliance, but we extend).
    \begin{enumerate}
        \item Under no time pressure [We find this]
        \item Under time pressure [We do not find this]
    \end{enumerate}
    
    \item There exists a trait that predicts overreliance rate. (We came up with this from pilot studies, where participants stated post-study that they either ignored or took into account AI, and we can predict that)
    \begin{enumerate}
        \item We can predict overreliance rate in second half of study from the first half.
    \end{enumerate}
    
    
    
    \item RQ: Do Big-5 / other traits (eg NFC or time pressure questions asked in advance) predict overreliance?
\end{enumerate}


% % OLD TEXT
%
% \begin{enumerate}
%
%     \item Time pressure impacts performance
%     \begin{enumerate}
%         \item Under time pressure, people spend less time per question. [We find this]
%         \item Different AI assistance is best in time-accuracy tradeoff. [We find this]
%         \item Overreliance rate increases under time pressure. [We find this for AI-before only, not AI-after or mixed.]
%     \end{enumerate}
%
%     \item Splitting people by overreliance rate
%     \begin{enumerate}
%         \item The first part of the study is indicative of whether a participant overrelies more or not. [We find this]
%         \item Not-overreliers and overreliers behave differently in terms of time and accuracy. [We often find this]
%         \item Not-overreliers and overreliers have best time-accuracy tradeoff with different AI assistance types. [Leave this until discussion? This is about adaptation.] [This is a complicated story: usually marginally true, not with statistical significance.]
%     \end{enumerate}
%
%     \item Within the mixed condition, performance on AI-before and AI-after is different to the pure conditions. (Cf scarcity effect.)
%     \begin{enumerate}
%         \item AI-before is different within mixed than pure AI-before. [Find this for no-time-pressure + overreliers only, rest is marginally true.]
%         \item AI-after is different within mixed than pure AI-after. [Find this for not-overreliers, and not true for overreliers?]
%         \item No-AI is different within mixed than pure No-AI. [We find this for not-overreliers under time pressure (and for overreliers under no time pressure?).]
%         \item Within the mixed conditions, there are different time-accuracy tradeoffs than the pure conditions. [We find this sometimes, especially after splitting into groups by overreliance rate.]
%         \item People overrely more in mixed condition than just AI-before or AI-after. [We find this when no time pressure, but this is not true when there is time pressure.]
%     \end{enumerate}
%
%     \item There is human-AI complementarity [We do not find this except for not-overreliers under time pressure]
%     \item A hypothesis about traits? Or just discussion? 
% \end{enumerate}






==> sections/old-4-problem-formulation.tex <==
%\section{Problem Formulation}

==> sections/old-5-experiment.tex <==
\section{Experiment}

\label{sec:experiments}

In this section, we describe the alien prescription task, the various design choices we made, and the procedure for the study we ran. 

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.9\textwidth]{figures/easy_alien_example}
    \caption{The alien prescription task, where participants must prescribe a single medicine. The information about the alien includes the alien's unique treatment plan (a set of rules) and the alien's observed symptoms. Participants have to use these observed symptoms and rules to prescribe a single medicine, such that only the observed symptoms and any potential intermediate (green) symptoms are used, and no other unobserved symptoms. When an AI assistance is shown, it is shown in a red box, like in this example. Here, the AI recommendation is the best possible (tranquilizers uses the most observed symptoms). 
    Vitamins is also a correct medicine, but is suboptimal as it uses fewer observed symptoms. 
    All other medicines are incorrect. 
    %Usually, there are two correct medicines per alien, with one being the best medicine (uses more observed symptoms), and the other the suboptimal medicine.
    }
    \label{fig:alien_example}
\end{figure*}

\subsection{Task Description}
We designed a task where users are asked to prescribe medicines to sick aliens, which we base on 
a the work of \citep{lage2019evaluation}. Our goal was to create a decision task that is accessible to laypeople but carries real-world resemblance.
Participants were shown a series of sick aliens for a fixed time of 20 minutes, corresponding to their `medical shift', and asked to prescribe a single medicine to each alien. 
By asking participants to act like doctors, and by emphasizing the importance of treating patients correctly, we aimed to motivate participants to obtain a high accuracy, while getting through as many sick patients as possible during their medical shift. 

\cref{fig:alien_example} shows an example of a single alien task. Based on observed symptoms and the `treatment plan' (which is a set of decision set rules unique to each alien), participants must decide a single medicine to give the alien. 
We chose decision sets as they are relatively easy for humans to parse~\cite{lakkaraju2016interpretable}. 
When we provide an AI assistance, we show it in a red box, as shown in \cref{fig:alien_example}. 
This box can provide both an AI recommendation and explanation (explanations are always an intermediate symptom that lead to the recommended medicine), and is provided before or after the participant's initial decision. 

We expanded on the setup in \citet{lage2019evaluation} in three ways. 
First, we always introduced intermediate symptoms to the task, which require participants to perform additional computation steps, and worked well as the explanation of an AI's recommendation.
Second, we allowed two possible correct medicines per alien. 
We defined the better medicine to be one that addressed more of the observed symptoms. 
Having a suboptimal medicine helps us to better analyze the role of overreliance on AI recommendations: suboptimal medicines are easily verified to be correct (even though they are not optimal), and so participants can overrely on them more easily than overrelying on a wrong recommendation. 

Third, we introduced two different difficulties of questions: easy and hard. 
We designed these such that easy questions require less cognitive effort for a human to find the best medicine, while hard questions require more computation. 
We ensured that both easy and hard questions superficially look very similar to a human, by having a similar length of lines, number of lines, and other visual aspects. 
%Further discussion and examples are in \cref{app:easy_hard_aliens}. 

% [Todo: justify why this task is sufficient / good for analysing results, even though the task is `made up'.]
While the task involves a fictional setting, it allows us to precisely manipulate the difficulty of the task, the optimality of the AI assistance, and the form of time pressure to understand how these factors impact human-decision making in settings where they must complete a large number of tasks in a short time.

\subsection{Conditions}
We consider four AI assistance types, and randomly assign participants to one of them.
\begin{enumerate}
    \item \textit{No-AI}: Do not provide any AI assistance. 
    \item \textit{AI-before}: An AI recommendation and explanation is provided to the participant along with the question, before the participant makes any decision.
    \item \textit{AI-after (/update)}: The participant makes an initial decision without any AI assistance. They are then provided with an AI recommendation and explanation, and allowed to change their initial answer. 
    \item \textit{Mixed}: Every question, the participant randomly gets one of the three above assistance types (No-AI, AI-before, AI-after). 
\end{enumerate}

We also randomly assign participants to have time pressure (with timers shown on the screen), or no time pressure (no timer on screen). 
These two conditions, combined with the four AI assistance types, leads to 8 participant conditions. 

Participants that do not have a timer see the screen in \cref{fig:alien_example}. 
Participants under time pressure had two timers on the screen: a global timer and a local timer. 
The global timer indicated the time remaining for participants to answer questions (start at 20 minutes and count down). 
The local timer is reset at the beginning of every question, and signifies the `recommended time' remaining to treat the specific alien patient. 
It starts at 1 minute. When it reaches 10 seconds, the color turns orange, and when it reaches 0 seconds, the color turns red (and the timer goes into negative numbers). 
For the AI-after assistance type, we give participants 20 seconds to respond to the AI input after they have made their initial decision. 
Although there was no requirement for participants to answer each question within the local timer's 60 seconds, the presence of the timer increases time pressure on the participant, which is increased as the timer changes color to orange and red.  The local timer allowed us to impose a type of time pressure that applied evenly to all parts of their shift, rather than participants feeling relaxed during the first part of their shift and increasingly pressured toward the end of their shift.

\subsection{Procedure}
Our study was conducted online on Prolific, a crowdsourcing platform. Before starting the main part of the study, participants had to accept a consent form, and then answer three pages of survey questions.
The first page asked demographic information, the second page asked 4 Need For Cognition trait questions and 2 questions about performance under time pressure, and the third page asked questions about their Big-5 Personality Traits (first 10 questions were the BFI-10 questions [ref], and last two were the two questions about neuroticism from BFI-S [ref]). 
Participants then had to read instructions/tutorial, and then successfully complete three practice questions (for which they had two attempts, similar to \citet{lage2019evaluation}: if they failed the first set of practice questions, they were given a second set of three questions). 

After completing the practice questions, the participants had 20 minutes to answer as many questions as possible. 
Approximately half of the questions participants saw were easy questions, and the other half hard questions. 

After the study, participants were shown a final screen where they were asked how helpful they found the AI assistance, what their strategy was (and if it changed when there was an AI input), and for any other feedback. 

\subsection{Participants}
We ran a study on 403 participants on Prolific. 
Only English speakers were allowed to participate. 
75 people failed the practice questions, and we removed a further 12 people for either answering questions too quickly (they spent less than 3 seconds on at least 3 questions), or taking much longer on one question than the rest (indicating they got distracted for one question). 
Our final results are based on the remaining 316 participants. 

[TODO: Stats about demographics]

Participants were paid \$7 for participating (median time was 37 minutes), and if they failed the practice questions, they were paid \$2 (their study ended immediately after failing the practice questions). 
We also incentivized participant performance by providing a bonus \$3 reward to the top-performing participant in each condition. 
%In general, we found that participants seemed to engage positively with the study, with many commenting that they had tried their best to treat their sick alien patients, and that they found the study was well-designed. 

\subsection{Design and Analysis}
We report three metrics.
\begin{enumerate}
    \item \textit{Accuracy}: if participants chose the \textit{best} medicine for the alien, we gave them a score of 1, a \textit{suboptimal} (but correct) medicine has a score of 0.5, and a \textit{wrong} medicine has a score of 0. We calculate the average accuracy over questions for each participant, and report mean and standard error across participants. 
    \item \textit{Response time}: we measure how long each participant takes to answer questions. We report the mean and standard error across participants. 
    \item \textit{Overreliance}: we define overreliance to be the proportion of times a participant gave the same answer as the AI when the AI was wrong or suboptimal \citep{buccinca2021trust, vasconcelos2023explanations}. 
    % \item \textit{Underreliance}: we define underreliance to be the proportion of times a participant gave a non-optimal answer when the AI was optimal.
\end{enumerate}

%[TODO-- state statistical tests used for comparisons]
Statistical tests used for comparisons (in note format currently). Our dependent variables are always accuracy (ordinal: 0, 0.5 or 1), response time, and overreliance rate.
\begin{enumerate}
    \item To compare across (the four) AI assistance types within time pressure or no-time pressure condition, we use analysis of variance, and then Tukey's HSD. We repeat this every time we compare across the AI assistance types (No-AI, AI-before, AI-after, mixed). We first find the average (mean) accuracy / response time / overreliance rate of each participant, and then conduct the tests on these averages.
    \item When comparing to AI-only accuracy (to make claims about complementarity), we do within-subject test to see if their accuracy (with AI) is greater than the AI's accuracy. We correct for multiple hypothesis tests using the Holm-Bonferroni method (correct for three comparisons, as three conditions (do not have a No-AI condition)). 
    % FDV: What is standard in HCI?  Do only correct within a "set" of results, and not across all the tests you run?  (Appropriate multiple hypothesis correction is nuanced; for now, let's do what is standard in the literature...)
    \item To compare between time pressure and no time pressure conditions, we conduct pairwise tests (time pressure or no time pressure) after fixing the AI assistance type (No-AI, AI-before, AI-after, mixed). We correct for multiple tests using the Holm-Bonferroni method (correct for four comparisons, as four conditions). 
    We do this when comparing between overreliers and not-overreliers too.
    \item When comparing performance of AI assistance types within the mixed condition, we ...
    \item When comparing performance of a specific AI assistance type within the mixed condition with the performance of the condition with only the AI assistance type (eg AI-before for mixed condition vs AI-before always), we use a mixed effect model, with participant as the random effect, and the fixed effects as: the condition (No-AI, AI-before, AI-after, mixed), the AI assistance type for the question (this can change only in the mixed condition), and the interaction of condition and AI assistance type. 
    Degrees of freedom: Kenward-Roger approximation.
\end{enumerate}



==> sections/old-6-results.tex <==
\section{Results}

% FDV: Can we make this into a statement e.g. time pressure impacts performance differentially based on assistance type, or is that not standard for IUI?
\subsection{The effect of time pressure on the performance of AI assistance types}

Summary: The existence of time pressure impacts which AI assistance types are better. 
(i) Participants speed up under time pressure, and No-AI accuracy also reduces. 
(ii) Accuracies are always similar across conditions, but AI-before becomes much faster under time pressure (overreliance rate also increases), so is better in the time-accuracy trade-off. 
(iii) Scarcity effect inside the mixed condition: AI-before is much faster than AI-after always, even when not under time pressure. AI-after is slower than the pure AI-after condition. Mixed's No-AI accuracy under time pressure is higher than pure No-AI (because participants are more motivated to do well as sometimes they see AI-before and AI-after too?). 
% (iv) Participants have higher accuracy on easy questions, and are quicker when no time pressure, but similar speed when there is time pressure. Many of the trends we saw earlier (eg AI-before is faster than AI-after and mixed) is on hard questions (only marginally quicker on easy questions). 
% FDV: Where is the easy vs. hard?  Or are you still adding plots? SS: I moved all discussion of easy vs hard to exploratory analysis section on adapting AI assistance type.

\begin{figure*}[th]
     
     \begin{subfigure}{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/Pareto no time pressure.PNG}
         \caption{Under no time pressure.}
         \label{fig:pareto_no_time_pressure}
     \end{subfigure}
     \begin{subfigure}{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/Pareto time pressure.PNG}
         \caption{Under time pressure.}
         \label{fig:pareto_time_pressure}
     \end{subfigure}
% FDV: I'm sure you're on this, but what the dashes and solids are is not in the legend
% FDV: These plots do a great job of showing the effect of mixed vs. not mixed.  I'm wondering if there's a way to also see more easily the effect of time pressure?  Right now, we have to look between the two plots and see that values in the 70s (left) become values in the 50s (right).
     \caption{Pareto plots: top left is desired (higher accuracy, lower response time per question). No time pressure vs time pressure. Under time pressure, AI-before becomes quicker. [Should I change the x-axis to be negative time, so that top right is desired, like normal Pareto frontier curves?]}
     \label{fig:pareto_effect_of_pressure}
\end{figure*}


Under no time pressure, AI-before, AI-after and mixed have similar accuracy and time. 
Under time pressure, AI-before is now quicker and has higher overreliance rate than AI-after and mixed, while all have similar acc [Done statistical analysis: ANOVA and Tukey's HSD].
See bold lines in \cref{fig:pareto_effect_of_pressure}
% TODO: check underreliance rates.

No time pressure: AI-before and AI-after greater than AI acc (70\%), but only marginally higher than No-AI acc. 
Time pressure: Same as AI acc (acc $\approx$ 70\%) [TODO: statistical analysis], but greater than No-AI acc. 

All conditions are much quicker under time pressure. 
Only AI-before's overreliance rate significantly increases under time pressure. 
No-AI has much worse accuracy under time pressure. [TODO: statistical analysis]
[Discussion] AI-before acc decreases marginally under time pressure: higher overreliance reduces acc, but lower underreliance makes up for this, meaning acc is not hurt too much. Also, relate to point a above.

Within mixed: AI-before always quicker than AI-after (NB this was not the case for the pure conditions when under no time pressure). [TODO: statistical analysis]

\textbf{Comparing mixed to pure conditions.}
Under no time pressure, AI-before marginally faster than pure [TODO: check if significant], and AI-after marginally slower [TODO: check if significant].
Under time pressure, AI-before same as pure, AI-after marginally slower than pure [TODO: check if significant].
Under no time pressure, No-AI is marginally faster than pure [TODO: check if significant], but same acc. Under time pressure, No-AI marginally slower than pure, but higher acc.



\subsection{A participant's overreliance rate is indicative of their performance}

Summary.
(i) Overreliers have lower accuracy and are usually quicker than not-overreliers. 
(ii) Can predict overreliance rate from first half of study for second half of study, and this predicts behavior too. 
(iii) Under no time pressure, earlier we saw that all conditions were similar (mixed has marginally lower accuracy), and within mixed, AI-before was significantly faster than AI-after. 
After splitting by overreliance rate, we see that not-overreliers have similar accuracy and time for all conditions, while overreliers have significantly lower accuracy on mixed. Within mixed, overreliers are significantly faster on AI-before (not-overreliers marginally faster / same response time). This helps explains the results seen in the earlier section. 
(iv) Under time pressure, earlier we saw that AI-before is quicker and has higher overreliance rate than AI-after and mixed, while all have similar accuracy. Mixed's No-AI was significantly better than pure No-AI. 
After splitting by overreliance rate, we see that overreliers contribute to the speed increase for AI-before: they are significantly quicker with AI-before (while not-overreliers are marginally quicker). 
Within mixed, we see a bigger difference in speed between overreliers than not-overreliers: overreliers' mixed has much faster AI-before than AI-after (but AI-after can marginally increase accuracy), while not-overreliers' mixed has marginally faster AI-before than AI-after (and same accuracy). 
Within mixed, we see that No-AI has higher accuracy than pure No-AI because of the not-overreliers, while overreliers' mixed No-AI is as low accuracy and quick as pure No-AI. 

Overreliers are at AI acc (70\%), and not-overreliers have greater than AI acc (>70\%). Under no time pressure, there is complementarity for not-overreliers, but under time pressure acc is no longer greater than human [TODO: statistically check if also greater than human-only acc]. 

\cref{fig:pareto_notime_overreliance}: 
Under no time pressure, overreliers have lower accuracy on mixed than others, and have higher overreliance rate on mixed than others (and marginally quicker). 
When looking inside mixed, this is because whenever participants see AI-before, they are very quick and have high overreliance (and low accuracy), as well as having low accuracy on No-AI. AI-after is similar to pure AI-after. 
Not-overreliers have similar performance, with higher accuracy than overreliers, on all conditions (marginal increase in accuracy for AI-before) [TODO: statistical analysis]. 
Mixed has a higher overreliance rate than AI-after. 

\cref{fig:pareto_time_overreliance}: 
Under time pressure, overreliers are quicker with AI-before than AI-after (not-overreliers are also quicker, but only marginally). 
Not-overreliers have higher accuracy than overreliers [TODO:statistical analysis]. 
Not-overreliers overrely on AI-before a significantly more than the AI-after and mixed, and overreliers only marginally overrely on AI-before more. 

Effect of time pressure is to speed up AI-before for both groups. Also increase overreliance on AI-before for both groups. [TODO: statistical analysis]

Not-overreliers significantly speed up under time pressure. Overreliers speed up on AI-before and mixed, and marginally speed up on AI-after. 

Within mixed, AI-before is always very quick regardless of time pressure. 
Mixed condition: for overreliers, AI-before is quicker than AI-after. For not-overreliers, only marginally quicker. (Regardless of time pressure.) 
Overreliers' mixed No-AI is low accuracy and quick as pure No-AI, while not-overreliers' mixed's No-AI has significantly higher accuracy (and marginally slower) than pure No-AI. 
[TODO: statistical analysis on this paragraph]

% FDV: Does it also make sense to show the timer versions of these?
\begin{figure*}[th]
     \begin{subfigure}{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/Pareto no time pressure overreliance low.PNG}
         \caption{Not-overreliers.}
         \label{fig:pareto_notime_overreliance_low}
     \end{subfigure}
     \begin{subfigure}{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/Pareto no time pressure overreliance high.PNG}
         \caption{Overreliers.}
         \label{fig:pareto_notime_overreliance_high}
     \end{subfigure}
     \caption{Pareto plots: top left is desired (higher accuracy, lower response time per question). Difference between overreliers and not-overreliers when there is no time pressure. }
     \label{fig:pareto_notime_overreliance}
\end{figure*}


\begin{figure*}[th]
     \begin{subfigure}{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/Pareto time pressure overreliance low.PNG}
         \caption{Not-overreliers.}
         \label{fig:pareto_time_overreliance_low}
     \end{subfigure}
     \begin{subfigure}{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/Pareto time pressure overreliance high.PNG}
         \caption{Overreliers.}
         \label{fig:pareto_time_overreliance_high}
     \end{subfigure}
     \caption{Pareto plots: top left is desired (higher accuracy, lower response time per question). Difference between overreliers and not-overreliers when there is time pressure. }
     \label{fig:pareto_time_overreliance}
\end{figure*}


Can use 10 mins to predict behavior of the two groups (overreliers and not-overreliers), showing overreliance is a stable trait. 
[Statistics: calculate confidence interval across r-value, and show >0?]


\subsection{Miscellaneous results: where should they go?}

Higher overreliance rate on AI-suboptimal than on AI-wrong. This is because the AI input is easy to verify. 
However, if we split people into two groups by overreliance rates on AI-suboptimal and then by AI-wrong, get very similar groups of people (I only looked at the performance of the groups). This indicates that it’s more about whether or not a person trusts the AI as a whole.
% FDV: This is interesting!

\textbf{Predicting performance from traits.}
Not much of significance (this in itself is a result): move to discussion?
Neuroticism does not seem to be a strong signal: 
(i) under no-timer, high neuroticism has higher no-AI acc and speed, 
(ii) high neuroticism marginally increases acc and is quicker (both timer and no-timer), 
(iii) high neuroticism people speed up more  under time pressure than low neuroticism. 
Under no-timer, high NFC people can be (marginally) slower and higher acc.
Under timer, high time-pressure-score has higher overreliance (even though they say they do better under time pressure). 


Easy vs hard questions:

\textbf{Easy vs hard questions.}
Under no time pressure, participants on easy questions have higher acc and are faster than on hard questions.
Under time pressure, participants on easy questions have higher acc than on hard questions, only marginally faster [TODO: check if significant]. 
Under time pressure, earlier we saw that AI-before was quicker than AI-after and mixed. This is only for hard questions: no such significant difference on easy questions (it’s marginal on questions aliens). [TODO: statistical analysis]

\textbf{Easy vs hard for the mixed condition.} %[Not sure if I should keep this, gets quite detailed. TODO: try to simplify.]
AI-before may not be significantly faster than AI-after on easy questions (regardless of time pressure), but is significantly faster on hard. [TODO: statistical analysis]
% Details: Under no time pressure, easy: AI-before acc now below pure, and time the same as pure; AI-after time slower than pure (and slower than AI-before). Hard: Accs all same, AI-before faster than pure (and faster than AI-after); other times same as pure (No-AI may be faster). 
% Under time pressure, easy: not much to say. Hard: AI-before slower than pure.

\textbf{Easy vs hard when split by overreliance rate.}
Under time pressure, overreliers on easy: AI-after better acc than AI-before. 
Under no time pressure, not-overreliers on hard: AI-after better acc than AI-before. 

\textbf{Easy vs hard for the mixed condition, split by overreliance rate.}
[Theory? AI-after can help overreliers (by slowing them down and increasing accuracy), but does not help not-overreliers (AI-before has same acc, but is same speed / quicker).]
Under no time pressure, overreliers can benefit from AI-after on easy questions, but always quicker with AI-before. Not-overreliers better/equal with AI-before always (AI-after does not help). 
Under time pressure, overreliers can benefit from AI-after on hard questions, but always quicker with AI-before. Not-overreliers better/equal with AI-before always (AI-after does not help, except maybe marginally increases acc on easy).



==> sections/old-7-discussion.tex <==
\section{Discussion and Conclusion}


% \subsection{What is the effect of time pressure in AI-assisted decision-making?}

% - Just by seeing a time pressured setting people's performance decreases overall, even when they are not under time pressure (Exp1). 
% - Different AI assistance are effective under time vs. no time pressure for different people (Exp 2).
% - Implications? We investigated time pressure but a similar effect to show under other types of pressure (e.g., stress etc CITE.) Given that these tools are increasingly being deployed in the workplace where people are under different types of pressure, it is important to understand the effectiveness of support in such pressured contexts and design support that adapts to the context. 

% \subsection{What individual differences may impact the effectiveness of different AI assistance under time pressure?}
% - We discovered that overreliance rate is stable throughout the duration of the study. And that it was a critical predictor of the effectiveness of different AI assistance.
% - However, unlike prior work, we did not observe overreliance rate to be significantly correlated with NFC. We suspect that this may partly due the task, which was game-like and inherently motivating. Thus even people low in NFC may have been motivated to cognitively engage with the task.
% - Further, we did not observe any strong correlation with the personality traits. Specifically, neuroticism has been shown by prior work to affect people's performance on tasks when under pressure. [What  is the correlation of overreliance and neuroticism under time pressure. I think the results state overall performance (under time pressure and no time pressure).] However, the measure of all the personality traits was based on a [few] questions rather than hundreds of questions that are typically administered for determining these traits. We therefore, cannot confidently assert that the lack of such correlation in our study is indeed due to lack of correlation of overreliance and personality traits.
% - Future work should investigate whether other contextual factors e.g., motivation to engage with the task or an interaction of multiple factors (stable traits and states) affect how people overrely on AI assistance.
% - Implications? We believe that to successfully adapt assistance to decision-makers we need to predict how that decision-maker will use the assistance. This can be done pre interaction with the system or in real time. We sought to understand if this overreliance trait could be captured beforehand (e.g., by personality variables), however support can be tailored as the person interacts with assistance and the system updates its priors on their usage of the assistance.

% \subsection{What are the opportunities for adaptive support under time pressure settings?}
% - Perhaps, scarcity effect results should come here.
% - Also bringing it all together the type of assistance and individual differences.


This work focusses on the accuracy-time tradeoff of different AI assistances, and how these change under time pressure. 
% Quick motivation of accuracy-time tradeoff and time pressure
Previous work compared different AI assistances focussing only on accuracy. %, with some recent works arguing that adapting the AI assistance is important. 
In this work, we consider response time to also be an important metric, such as when using AI assistance in time-pressured scenarios, or scenarios where we hope the AI assistance will speed up human decision-making. 
We specifically consider the setting where people are under time pressure (such as making decisions in an emergency room~\citep{patel2008translational,franklin2011opportunistic,rundo2020recent}), where the accuracy-time tradeoff is particularly important. 
Some recent works have shown benefits of adapting the AI assistance to maximise accuracy~\citep{noti2022learning,ma2023who,bhatt2023learning}, and we are interested in doing the same for the accuracy-time tradeoff. 

% First key result
We find that introducing time pressure can change the accuracy-time tradeoff between different AI assistances, making our AI-before condition significantly faster than the AI-after and mixed conditions.

\subsection{Participant behaviour changes after they experience time pressure on the task}

% Experiment 1 then 2
In our first experiment (\cref{sec:experiment1}), we alternately put the same participant under time pressure and not under time pressure.
However, we found that once a participant had been under time pressure once, their performance remained similar even if they were not under time pressure later in the study. 
Further work is required to investigate why the same person's behaviour changes after they experience time pressure on the task: they appear to learn how to perform the task quickly, and retain this behaviour, even if that reduces accuracy. 

We should therefore only compare AI assistances to each other within the setting of interest (whether or not there is time pressure).
We cannot necessarily draw conclusions about the no-time-pressure setting after putting the same participant under time pressure. 
We therefore designed a second experiment (\cref{sec:experiment2}) where each participant was either under time pressure or not. 
This design is also more similar to studies in current literature, where participants have no time pressure throughout the study. 

\subsection{The interaction between overreliance and time pressure}

We argue that overreliance is important, and we investigate how this interacts with time pressure. 
Appropriate reliance is especially important in time-pressured scenarios: we want to encourage a person to follow a correct AI suggestion in order to save time; conversely, when the task is more difficult and the AI assistant may be incorrect, we may want to slow down the person to ensure they still make the correct decision. 
Appropriate reliance is also important to achieve human-AI complementarity~\citep{bussone2015role, lai2019human, jacobs2021machine}. 
Previous work has argued that overreliance (or reliance) on AI can vary between different AI assistances and conditions: %, and increasing appropriate reliance is important: in order to achieve human-AI complementarity, participants must have low overreliance on AI assistances (and high reliance when the AI is correct) [refs]. 
%Previous studies have found that 
AI assistances that force people to slow down and cognitively engage with the AI assistance (like AI-after) can reduce overreliance \citep{buccinca2021trust}, and when an AI assistance is shown less often (like when adaptively showing AI assistances), people rely on it more (the scarcity effect) \citep{noti2022learning}. 
% Like these previous works, we also find that overreliance is important, and we investigate how these effects interact with time pressure. 

%We hypothesise that we will see the scarcity effect both not under time pressure (like in \citet{noti2022learning}), and under time pressure. 
We observe the scarcity effect when there is no time pressure (like in \citet{noti2022learning}), but find that the scarcity effect disappears under time pressure. 
Participants already overrely more on the AI when under time pressure, and the scarcity effect does not compound with this increased overreliance. 
In our setting, participants experienced fairly strong time pressure: it is possible that, under less time pressure, there may still be a (smaller) scarcity effect. 

We also hypothesise that different people have different tendencies to overrely, and find evidence that this is true. 
%While previous works focus on how different AI assistances impact overreliance, we also hypothesise that different people have different tendencies to overrely, and that there is some underlying trait that predicts a person's overreliance rate. 
We base this hypothesis from our pilot studies, where many participants (after the study) said that they either ignored the AI input, or relied heavily on it. 
There is also evidence in medical settings that experts with less experience trust AI more than experts with more experience~\citep{gaube2021ai,bayer2022role}, and this may also result in different overreliance rates. 
Although we are able to predict participants' overreliance behaviour in the later part of our studies from earlier, we find only marginal correlations between overreliance behaviour and personality traits (Big-5 Personality Traits, NFC, and self-reported belief of performance under time pressure). 
%We find evidence that our hypothesis is true: we split people by their tendency to overrely, and find that we can predict their overreliance behaviour in the later part of our studies from earlier. 
%However, when we try to predict a person's tendency to overrely based on personality trait questions asked at the beginning of the study (Big-5 Personality Traits, NFC, and self-reported belief of performance under time pressure), we only find marginal correlations.
Previous work has argued that Agreeableness and Conscientiousness may be related to trust in AI systems and~\citep{riedl2022trust}, but we do not find significant evidence of this in our setting. 
Further work is required to investigate the relationship between overreliance and personality traits in more detail. 

We find that overreliers and not-overreliers behave differently with AI assistances, suggesting that it may be useful to consider them independently when adapting AI assistances (\cref{sec:exploratory-adapting}). 
The group that does not overrely achieves human-AI complementarity (higher accuracy than both No-AI and AI-only), while being slower than the group that overrelies. 
The two groups benefit differently from different AI assistance types (which is made especially clear after we separately analyse performance on easy and hard questions), suggesting that adapting the AI assistance to a person's overreliance rate can be beneficial. 
For example, we can increase the accuracy of overreliers by slowing them down with AI-after assistance on hard questions, while showing AI-after to not-overreliers does not significantly increase accuracy (and only slows them down). 

Future work could investigate why these two groups of people behave differently, and look at the different mechanisms they might be using. 
For example, are not-overreliers using AI assistance as a guide to check information, before making their own decision? 
Such mechanisms are likely to also depend on the specific task. 

\subsection{Limitations}

In our experiments, participants had to complete a series of logic puzzles, where all information was shown on the screen. 
This allowed us to precisely manipulate the difficulty of the task (such as by having easy and hard questions), the optimality of the AI assistance, and the form of time pressure. 
However, a key limitation of our work is that such a setting may not be realistic: in many real settings, prior knowledge of aspects of the task is important. 
Because the logic puzzles are new and different, participants may always be in System II thinking~\cite{kahneman2011thinking}, reducing the effect of cognitive forcing functions like AI-after (previous work has argued AI-after reduces overreliance because it can push people from System I to System II thinking \citep{buccinca2021trust}). 
Additionally, our task is in a non-critical setting, unlike other realistic time-pressured scenarios like doctors in emergency rooms~\citep{patel2008translational,franklin2011opportunistic,rundo2020recent}. 
Previous work has suggested that experts may have similar behaviour as participants in crowd-based studies~\citep{gaube2021ai}, but we do not know if this will also hold under time pressure. 

The AI explanation that we showed participants (along with the AI recommendation) in our setting was an intermediate symptom that led to the AI recommendation, and was easily verifiable. 
This verifiability might impact how people use AI assistances~\citep{fok2023search}.
Different forms of AI explanations may lead to different results. 
We also only compared two forms of AI assistance (AI-before and AI-after). We chose these because AI-before is widely-used, and AI-after can slow people down and potentially reduce overreliance. 
Future work could consider how people act under time pressure with other AI assistance types. 
For example, does providing only an AI recommendation (without an explanation) lead to similar results? Do other cognitive-forcing functions like ``on-demand''~\citep{buccinca2021trust} lead to similar accuracy-time tradeoffs as AI-after under time pressure? 

% % SS: Not including this because I am unsure what exactly to say.
% We allowed our AI recommendations to be right, suboptimal but correct, and wrong. 
% This made it easy to overrely on the AI when the AI was suboptimal but correct, and we did see higher reliance on suboptimal AI recommendations than wrong AI recommendations. 





% \subsection{Miscellaneous results}

% Higher overreliance rate on AI-suboptimal than on AI-wrong. This is because the AI input is easy to verify. 
% However, if we split people into two groups by overreliance rates on AI-suboptimal and then by AI-wrong, get very similar groups of people (I only looked at the performance of the groups). This indicates that it’s more about whether or not a person trusts the AI as a whole.
% % FDV: This is interesting!
% 
% \textbf{Predicting performance from traits.}
% Not much of significance (this in itself is a result): move to discussion?
% Neuroticism does not seem to be a strong signal: 
% (i) under no-timer, high neuroticism has higher no-AI acc and speed, 
% (ii) high neuroticism marginally increases acc and is quicker (both timer and no-timer), 
% (iii) high neuroticism people speed up more  under time pressure than low neuroticism. 
% Under no-timer, high NFC people can be (marginally) slower and higher acc.
% Under timer, high time-pressure-score has higher overreliance (even though they say they do better under time pressure). 

